Probabilistic Bisimulation for Parameterized Systems (Technical Report)

Probabilistic bisimulation is a fundamental notion of process equivalence for probabilistic systems. Among others, it has important applications including formalizing the anonymity property of several communication protocols. There is a lot of work on verifying probabilistic bisimulation for finite systems. This is however not the case for parameterized systems, where the problem is in general undecidable. In this paper we provide a generic framework for reasoning about probabilistic bisimulation for parameterized systems. Our approach is in the spirit of software verification, wherein we encode proof rules for probabilistic bisimulation and use a decidable first-order theory to specify systems and candidate bisimulation relations, which can then be checked automatically against the proof rules. As a case study, we show that our framework is sufficiently expressive for proving the anonymity property of the parameterized dining cryptographers protocol and the parameterized grades protocol, when supplied with a candidate regular bisimulation relation. Both of these protocols hitherto could not be verified by existing automatic methods. Moreover, with the help of standard automata learning algorithms, we show that the candidate relations can be synthesized fully automatically, making the verification fully automated.

==> algorithm.tex <==
\section{The Algorithm}
\label{sec:algorithm}
In this section, we describe how to verify a probabilistic bisimulation for an MDP
under some restrictions. The idea is that when an MDP is bounded-branching
with a finite number of distinct transition probabilities, the verification
condition may be expressed with a finite number of first-order formulas.



\begin{alignat*}{3}
&\forall p. 			    		       	&& (p,p) \in R,\\
&\forall p. \forall q.    			    && (p,q) \in R\to (q,p)\in R,\\
&\forall p. \forall q. \forall r.\	&& (p,q) \in R \wedge ((q,r)\in R \to (p,r)\in R).
\end{alignat*}
Define $S_a(p,q) = \{s\in S: \delta_a(p,s) > 0 \vee \delta_a(q,s) > 0 \}$.
Let $\mathcal S_a(p,q)$ denote the projection of $S/R$ on $S_a(p,q)$.
That is, $\mathcal S_a(p, q) =
\{ S'\cap S_a(p,q) : S' \in S/R \}$.
Note that $|\mathcal S_a(p,q)|\le 2N$.
Define formula $\phi_R(p,q,a,\rho)$ as
$$
\forall S \in \mathcal S_a(p,q).\ 
(\sum_{s\in S} \delta_a(p,s) = \sum_{s\in S} \delta_a(q,s) = \rho).
$$
%Note that this is only a sufficient condition, as it actually checks that
%$p \tran{\rho}_a S \Leftrightarrow q \tran{\rho}_a S$ over all possible partition $S$.
Now, to verify that $R$ is a probabilistic bisimulation, it suffices to check that 
\begin{eqnarray}\label{alg:vc}
(\bigwedge_{\psi\in\Psi} \psi ) \wedge
(\forall (p, q)\in R.\ \forall a\in \ACT.\ \exists \rho\in\mathcal P.\ \phi_R(p,q,a,\rho))
\end{eqnarray}
holds. To check it, given $(p,q)\in R$, we first guess the configurations reachable from
$p$ and $q$. Then we guess the transition probabilities from $p$ and $q$

==> conc.tex <==
\section{Conclusion}
\label{sec:conc}
\OMIT{
In this paper, we have described the framework of regular relations (i.e.
the decidable first-order theory over the universal automatic structure) for 
modelling
infinite-state probabilistic transition systems (PTS) and reasoning
about probabilistic bisimilarity for these systems.
}
\OMIT{
While we focus on proof rules
for probabilistic bisimulation, our setting provides a general \emph{regular model
checking} framework for probabilistic systems. 
Our framework leads to a fully-automatic procedure 
for  regular probabilistic bisimulation for regular PTS.
}
\OMIT{
We have shown that the regular framework is sufficiently powerful
to capture the proofs of the anonymity property of the parameterized
dining cryptographers protocol and of the parameterized grades protocol. To the 
best 
of our knowledge, the universal automatic structure is the first decidable 
theory that can express such proofs. Finally, we have also shown that with the
help of standard learning algorithms, some of these proofs could be
fully-automatically synthesized.
}
%apply \mbox{SAT-based} enumerations and 
%\cite{LR16,Vardhan-thesis,HV05,CHLR17,Neider13,NT16,GNMR16,LMN16} for
%efficiently enumerating candidate regular probabilistic bisimulation for a given
%regular probabilistic transition system.
\OMIT{
An immediate future avenue is to study a more scalable proof enumeration
strategy that could be successful in the case of the grades protocol.
We would like to address the
issue of unbounded numerical data for each process; this issue prevents us from
applying our technique in this paper to examples such as the grade
protocol in \cite{KMOWW11}.
}


==> model-symbols.tex <==
\subsection{Probabilities as symbols}\label{sec:prob-as-sym}
Let $\struct :=\transysMDP$ be a bounded-branching MDP
with finitely many transition probabilities.
Suppose we are given an equivalence relation $R$
as a candidate of probabilistic bisimulation for $\struct$.
To verify that $R$ satisfies~(\ref{defn:pb-proof-rule}),
we construct a first-order formula that
i) guesses the set $S'$ of configurations reachable from
$p$ and $q$ in one step;
ii) guesses the transition probabilities from $p$ and $q$
to the configurations in $S'$;
iii) guesses the partitioning of $S'$
induced by the equivalence $R$;
iv) checks that the sums of the transition probabilities
from $p$ and $q$ to that partitioning
satisfy the constraints given in~(\ref{defn:pb-proof-rule}).
These guesses and checks can be encoded in one single
sentence by enumerating all possible cases via disjunction.

For example, the fact that a configuration
$p$ can reach exactly three configurations via action $a$
can be expressed as
\begin{eqnarray*}
\begin{split}
& \exists u_1,u_2,u_3 \in S.\ \exists p_1, p_2, p_3\in P(\struct).\ \\
& \quad (u_1\neq u_2 \wedge u_2 \neq u_3 \wedge u_3 \neq u_1 \wedge
p\tran{p_1}_a u_1 \wedge p\tran{p_2}_a u_2 \wedge p\tran{p_3}_a u_3\\
& \quad\ \wedge\ \forall u\in S.\ (u = u_1 \vee u = u_2 \vee u = u_3 \vee
(\forall \rho \in P.\ \neg (p \tran{\rho}_a u)))).
\end{split}
\end{eqnarray*}
Consider another configuration $q \in S$
that can reach exactly two configurations via 
$q\tran{q_1}_a v_1$ and $q\tran{q_2}_a v_2$.
If $(p,q)\in R$ and $R$ is a probabilistic bisimulation,
then~(\ref{defn:pb-proof-rule}) must hold on the partitioning of 
$S' := \{u_1,u_2,u_3,v_1,v_2\}$ induced by the equivalence $R$.
To check this, we can disjunct formulas 
corresponding to each possible partitioning of $S'$
and assert that~(\ref{defn:pb-proof-rule}) should hold for a partitioning
if that partitioning is induced by $R$.
For example, the fact that~(\ref{defn:pb-proof-rule}) holds for
partitioning $\{\{u_1,v_1\},\{u_2, u_3, v_2\}\}$
can be checked with
\begin{eqnarray*}
    R(u_1,v_1) \wedge R(u_2,u_3) \wedge R(u_3,v_2)
    \wedge p_1=q_1 \wedge p_2+p_3=q_2.
\end{eqnarray*}
Observe that we only need five parameters
to construct a first-order formula carrying out
the guesses and checks described above,
namely, a pair of configurations ($p$ and $q$ here),
an action ($a$ here), and the numbers of configurations
the two configurations can reach via that action (3 and 2 here).
We shall denote this formula as $\varphi(p,q,a,n,m)$.

More precisely, we define
\begin{equation}
\begin{split}
    \varphi(p,q,a,n,m) :=\ & (n = 0 \vee m = 0 \Rightarrow n = m \wedge \varphi_0(p,a) \wedge \varphi_0(q,a))\\
    & \quad \wedge (n \neq 0 \wedge m \neq 0 \Rightarrow \varphi_1(p,q,a,n,m)),
\end{split}
\end{equation}
where $\varphi_0(s,a) := \forall s' \in S.\ \neg (s \to_a s')$
means that configuration $s$ cannot move to any configuration through action $a$.
To specify $\varphi_1$,
let $\mathcal P := \{\{p_1,...,p_n, q_1,...,q_m\} : p_i,-q_j\in P(\struct)$
for $1\le i \le n$ and $1\le j \le m\}$ 
be a collection of \emph{multi-sets} where each multi-set has cardinality $n+m$.
Let $\mathcal P'$ denote the collection of partitioning
of the multi-sets in $\mathcal P$, such that
for each partitioning $\mathcal Q\in \mathcal P'$,
$$
\sum\nolimits_{p_i \in Q \wedge p_i>0} p_i = -\sum\nolimits_{q_i \in Q \wedge q_i<0} q_i
\quad\mbox{for each partition $Q \in \mathcal Q$.}
$$
%Finally, define $\mathcal{P''}=\{\bigcup_{Q\in  \mathcal Q} Q : \mathcal Q \in \mathcal P'\}$.
%Note that $\mathcal{P''}$ is a subset of $\mathcal{P}$ and
Note that $\mathcal{P'}$ is a finite set
computable solely from $P(\struct)$ and parameters $n$ and $m$.
The formula $\varphi_1(p,q,a,n,m)$ is then defined as 
$$
\varphi_1(p,q,a,n,m) := 
\bigvee\nolimits_{\mathcal Q\in \mathcal P'} \varphi_2(p,q,a,n,m,\mathcal Q),
$$
where the formula $\varphi_2(p,q,a,n,m,\mathcal Q)$ is given as follows:
\begin{equation}
\begin{split}
& \exists u_1,...,u_n, v_1,...,v_m \in S.\\
& \quad \wedge (\forall u\in S.\ (p \to_a u) \Rightarrow u = u_1 \vee \cdots \vee u = u_n)\\
& \quad \wedge (\forall v\in S.\ (q \to_a v) \Rightarrow v = v_1 \vee \cdots \vee v = v_m)\\
& \quad \wedge \left(\bigwedge\nolimits_{1\le i<j\le n} u_i \neq u_j \right)
   \wedge \left(\bigwedge\nolimits_{1\le i<j\le m} v_i \neq v_j \right)\\
& \quad \wedge \left(\bigwedge\nolimits_{Q \in \mathcal Q} \bigwedge\nolimits_{p_i \in Q \wedge p_i>0} (p\tran{p_i}_a u_i)\right)\\
& \quad \wedge \left(\bigwedge\nolimits_{Q \in \mathcal Q} \bigwedge\nolimits_{q_i \in Q \wedge q_i<0} (q\tran{-q_i}_a v_i) \right)\\
& \quad \wedge \left(\bigwedge\nolimits_{Q \in \mathcal Q} \bigwedge\nolimits_{p_i,p_j \in Q \wedge p_i,p_j>0} R(u_i,u_j)\right)\\
& \quad \wedge \left( \bigwedge\nolimits_{Q \in \mathcal Q} \bigwedge\nolimits_{q_i,q_j \in \mathcal Q \wedge q_i,q_j<0} R(v_i,v_j) \right).
\end{split}
\end{equation}
Hence, $\varphi(p,q,a,n,m)$ is true if and only if configurations $p$ and $q$
have non-zero transition probabilities to \emph{exactly} $n$ and $m$
configurations, respectively, via action $a$, such that
$p \tran{\rho}_a S' \Leftrightarrow q \tran{\rho}_a S'$ for all $S' \in S/R$ and $\rho>0$.
We summarize the discussion so far in the following proposition.
\begin{proposition}\label{prop:prob-as-symbols-proof-rule}
    Let $\struct := \transysMDP$ be an MDP
    where the branching is bounded by $N$
    and the number of distinct transition probabilities is finite.
    Given an equivalence $R$ over $S$,
    define formula $\varphi(p,q,a,n,m)$ as described above.
    Then $R$ is a probabilistic bisimulation for $\struct$ if and only if
\begin{eqnarray}
\forall (p,q)\in R. \left(\bigwedge\nolimits_{a \in \ACT} 
\bigvee\nolimits_{n,m \in \NatInt{0}{N}}  \varphi(p,q,a,n,m) \right).
\end{eqnarray}
\end{proposition}
For each $a\in \ACT$ and $\rho\in P(\struct)$,
let $R_{a,\rho}\subseteq S \times S$ be a relation
so that $(p,q)\in R_{a,\rho}$ iff $p \tran{\rho}_a q$.
Since first-order theory is decidable on automatic structures,
the following result is immediate:
\begin{corollary}
    Verifying regular probabilistic bisimulation for an MDP $\struct$
    is decidable if i) $\struct$ is bounded-branching,
    ii) the number of the transition probabilities of $\struct$ is finite,
    and
    iii) $\{R_{a,\rho} : a\in\ACT, \rho\in P(\struct)\}$ is a set of regular relations.
\end{corollary}
